Integrating deduction and model finding in a language independent setting

Software artifacts are ubiquitous in our lives being an essential part of home appliances, cars, cel phones, and even in more critical activities like aeronautics and health sciences. In this context software failures may produce enormous losses, either economical or, in the extreme, in human lives. Software analysis is an area in software engineering concerned on the application of different techniques in order to prove the (relative) absence of errors in software artifacts. In many cases these methods of analysis are applied by following certain methodological directives that ensure better results. In a previous work we presented the notion of satisfiability calculus as a model theoretical counterpart of Meseguer's proof calculus, providing a formal foundation for a variety of tools that are based on model construction. The present work shows how effective satisfiability sub-calculi, a special type of satisfiability calculi, can be combined with proof calculi, in order to provide foundations to certain methodological approaches to software analysis by relating the construction of finite counterexamples and the absence of proofs, in an abstract categorical setting.

==> dedication.tex <==
%!TEX root = analysis.tex

\section{Dedicated to Tom\'{a}s Esteban Eduardo Maibaum in his 70th.+ birthday}
\label{dedication}
This dedication is being written by me (Carlos {G.} Lopez Pombo), on behalf of the authors of this paper. The joke of calling Tom by the Spanish translation of his names (the amount of which would certainly fit the latin tradition) was never funny, and after some time I realised that it was not meant to be as he is one of us. Tom was born in Hungary and left with his family being a kid, in the aftermath of WWII; he was raised in Canada, where he grew, and got a degree in pure mathematics from the University of Toronto; he moved to England where he got a PhD in computer science from Queen Mary and Royal Holloway, Colleges of the University of London. Held academic positions in King's College and Imperial College and in both places was appointed head of the department of computer science. Returned to Canada where he still hold the position of Tier I Canada Research Chair in the Foundations of Software Engineering and is Emeritus Professor in the Department of Computing and Software at McMaster University. None of the preceding data really matters because he is one of us; not even his passionate love for soccer, entangled with his ragging hate towards Maradona and Argentina's futbol team counts; he is one of us. 

Anyone can tell that he is not really Hungarian, Canadian or English; he gives hugs and kisses, opens his home, shares his table and most notably, jokes about the type of things that polite people would never dare mention, to then, laugh about it in your face; he is the kind of generous and loving Argentinian friend anyone would pray to have.\\

In 2010 I already had a couple of papers with Tom but never had really worked with him. I met him in person for the first time in Natal, Brasil, for ICTAC 2010 (there might be some dispute whether he is one of us or one of them, a part of Tom's heart is certainly Carioca, not necessarily Brazilian). There, we had long discussions about formal specification of software systems over countless \emph{chope}; it would take a couple of years for me to understand how much he hated our joint paper accepted in that conference. As I mentioned in the introduction, Tom and Institutions are not a match. Nonetheless, he invited me to visit him in Canada and, six month later, I was heading to Canada to work with him for the first time. There was never a discussion, I was staying at his place, as his kind and generous heart always dictate. There, I met Jan, his wife, and part of my admiration for Tom's amazing work in computer science shifted to Jan's cooking. I visited Tom and Jan many times over the years, at the beginning in Canada, and nowadays in England, where they currently live. Mum and dad are the lawful nicknames they won for their warm kindness and caring. Luckily for me, Tom like me a lot more than how much he hates the papers I forced him to coauthor with me.



